Minimum Word Error Rate Training for Attention-based Sequence-to-Sequence Models

Sequence-to-sequence models, such as attention-based models in automatic speech recognition (ASR), are typically trained to optimize the cross-entropy criterion which corresponds to improving the log-likelihood of the data. However, system performance is usually measured in terms of word error rate (WER), not log-likelihood. Traditional ASR systems benefit from discriminative sequence training which optimizes criteria such as the state-level minimum Bayes risk (sMBR) which are more closely related to WER. In the present work, we explore techniques to train attention-based models to directly minimize expected word error rate. We consider two loss functions which approximate the expected number of word errors: either by sampling from the model, or by using N-best lists of decoded hypotheses, which we find to be more effective than the sampling-based method. In experimental evaluations, we find that the proposed training procedure improves performance by up to 8.2% relative to the baseline system. This allows us to train grapheme-based, uni-directional attention-based models which match the performance of a traditional, state-of-the-art, discriminative sequence-trained system on a mobile voice-search task.

==> related_work.tex <==
\section{Related Work}
\label{sec:related-work}
Discriminative sequence training of acoustic models is a well-studied problem in
the context of traditional ASR systems.
Examples of such approaches include maximum mutual information
(MMI)~\cite{BahlBrowndeSouzaEtAl86}, minimum phone error (MPE)~\cite{Povey03},
and the state-level minimum Bayes risk (sMBR)~\cite{KaiserHorvatKacic00,
PoveyKingsbury07}.
State-of-the-art ASR systems are typically first trained to optimize either a
cross-entropy of CTC criterion before discriminative sequence training to
optimize criteria such as sMBR~\cite{Kingsbury09, VeselyGhoshalBurgetEtAl13,
SakVinyalsHeigoldEtAl14}.

In the context of sequence-to-sequence models, there have been a few previous
proposals to optimize task-specific losses.
In their seminal work, Graves and Jaitly~\cite{GravesJaitly14} minimize expected
WER of an RNN-T model by approximating the expectation with samples drawn from
the model.
This approach is similar to the edit-based minimum Bayes risk (EMBR) approach
proposed by Shannon, which was used for minimum expected WER training of
conventional ASR systems~\cite{Shannon17} and the recurrent neural
aligner~\cite{SakShannonRaoEtAl17}.
An alternative approach is based on reinforcement learning, where the label
output at each step can be viewed as an \emph{action}, so that the task of
learning consists of learning the \emph{optimal policy} (i.e., optimal output
label sequence) which results in the greatest reward (lowest expected
task-specific loss).
Ranzato et al.~\cite{RanzatoChopraAuliEtAl16} apply a variant of the REINFORCE
algorithm~\cite{Williams92} to optimize task-specific losses for summarization
and machine translation.
More recently Bahdanau et al.~\cite{BahdanauBrakelLoweEtAl17} use an
actor-critic approach, which was shown to improve BLEU scores for machine
translation.
%that uses a separate critic network to estimate the
%expected reward of a particular action,

Our proposed approach is similar to ~\cite{GravesJaitly14, Shannon17} in that we
approximate the expected WER using hypotheses from the model.
However, unlike Sak et al.~\cite{SakShannonRaoEtAl17} we find that the process
is more effective if we approximate the expectation using N-best hypotheses
decoded from the model using beam-search~\cite{SutskeverVinyalsLe14} rather than
sampling from the model (See section~\ref{sec:results1}).

